Is There a One-Model-Fits-All Approach to Information Extraction? Revisiting Task Definition Biases

Definition bias is a negative phenomenon that can mislead models. Definition bias in information extraction appears not only across datasets from different domains but also within datasets sharing the same domain. We identify two types of definition bias in IE: bias among information extraction datasets and bias between information extraction datasets and instruction tuning datasets. To systematically investigate definition bias, we conduct three probing experiments to quantitatively analyze it and discover the limitations of unified information extraction and large language models in solving definition bias. To mitigate definition bias in information extraction, we propose a multi-stage framework consisting of definition bias measurement, bias-aware fine-tuning, and task-specific bias mitigation. Experimental results demonstrate the effectiveness of our framework in addressing definition bias. Resources of this paper can be found at https://github.com/EZ-hwh/definition-bias

==> Table/incontextcase.tex <==
\begin{table*}[!htb]
    \centering
    \begin{tabular}{p{0.15\textwidth}p{0.82\textwidth}}
        \toprule
        \colorbox{lightgray}{\textbf{Instruction}} &  \textit{Given a phrase that describes the "\underline{publication date}" relationship between two words, extract the subject and object that describe the relationship. The output format should be ```(subject1, object1), (subject2, object2)```}\\
        \midrule
        \textbf{Demonstration} & \textbf{Input:} \textit{Priyapetta Kukku is a 1992 Malayalam film written and directed by Sunil.} \textbf{Output:} \textit{(Priyapetta Kukku, 1992)}\\
        & ......\\
        \midrule
        \colorbox{lime}{\textbf{Extraction}} & \textbf{Input:} \textit{"Baby It's Christmas" is a song recorded by British girl group Bananarama, released on 13 December 2010 as a digital EP in the UK and most European territories.} \\
        & \textbf{Output:} \textit{(Baby It's Christmas, 13 December 2010)}\\
        \bottomrule
    \end{tabular}
    \caption{The formats of input and output of in-context Relation Extraction.}
    \label{tab:my_label}
\end{table*}

==> Table/main_result_compare.tex <==

\begin{table}[!ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
        \textbf{Dataset} & Finetuning & Weighted & Origin + LoRA & Ours \\
    \midrule
        ACE 04 & 71.22 & 71.73 & 78.42 & 79.07 \\
        ACE 05 & 71.80 & 70.71 & 79.79 & 78.88  \\
        CoNLL 03 & 83.63 & 86.27 & 90.85 & 91.26 \\
        Ontonotes & 64.82 & 69.93 & 85.89 & 86.08 \\
        WikiANN en & 58.18 & 58.81 & 86.52 & 86.36\\
        TweetNER 7 & 58.93 & 56.40 & 59.39 & 58.68\\
        WikiNeural & 49.94 & 58.49 & 92.40 & 92.73\\
        PolyglotNER & 39.69 & 54.15 & 70.85 & 71.41 \\
    \midrule
        CoNLL 04 & 49.33 & 46.36 & 66.41 & 65.42 \\
        NYT10 & 70.37 & 68.35 & 82.78 & 82.37 \\
        NYT11 & 44.41 & 45.17 & 54.28 & 54.81 \\
        GIDs & 61.69 & 63.88 & 76.22 & 77.32 \\
        WikiKBP & 36.22 & 34.74 & - & \\
    \bottomrule
    \end{tabular}}
    \caption{Main result for comparing with other models on NER and RE tasks.}
    \label{tab:main_result_comp}
\end{table}
